Artificial diffusion for convective and acoustic low Mach number flows I: Analysis of the modified equations, and application to Roe-type schemes

Three asymptotic limits exist for the Euler equations at low Mach number - purely convective, purely acoustic, and mixed convective-acoustic. Standard collocated density-based numerical schemes for compressible flow are known to fail at low Mach number due to the incorrect asymptotic scaling of the artificial diffusion. Previous studies of this class of schemes have shown a variety of behaviours across the different limits and proposed guidelines for the design of low-Mach schemes. However, these studies have primarily focused on specific discretisations and/or only the convective limit. In this paper, we review the low-Mach behaviour using the modified equations - the continuous Euler equations augmented with artificial diffusion terms - which are representative of a wide range of schemes in this class. By considering both convective and acoustic effects, we show that three diffusion scalings naturally arise. Single- and multiple-scale asymptotic analysis of these scalings shows that many of the important low-Mach features of this class of schemes can be reproduced in a straightforward manner in the continuous setting. As an example, we show that many existing low-Mach Roe-type finite-volume schemes match one of these three scalings. Our analysis corroborates previous analysis of these schemes, and we are able to refine previous guidelines on the design of low-Mach schemes by including both convective and acoustic effects. Discrete analysis and numerical examples demonstrate the behaviour of minimal Roe-type schemes with each of the three scalings for convective, acoustic, and mixed flows.

==> abstract2.tex <==
%TC:ignore
\noindent \textbf{Paper II: Application to AUSM, Zha-Bilgen and Toro-Vasquez flux splitting schemes}
%TC:endignore

\noindent AUSM family schemes are popular for low Mach number simulations, but past numerical analysis studies tend to focus only on a single scheme, and often neglect flow with acoustic effects.
In our recent paper **\textit{Hope-Collins \& di Mare, JCP 2021}**, we derived constraints on the artificial diffusion of low Mach number schemes for flows both with and without acoustic effects.
By forming an approximate diffusion matrix in the entropy variables for the AUSM family, as well as the closely related Zha-Bilgen (ZB) and Toro-Vasquez (TV) families of schemes, we can apply these constraints to derive and analyse the required form of each family at low Mach number.
We confirm the causes of two previously reported instabilities, and show a \mathcalOM{2} CFL bound for AUSM$^+$-up.
Numerical examples confirm these results, and show \emph{?`?`differences $x$ and $y$ between the families??}.
These results give clear guidelines for designing future low Mach number AUSM/ZB/TV schemes, as well as improving existing schemes.

==> appendices/asymptotic_notation.tex <==
The standard definition of big-O ($\mathcal{O}$) is as an upper bound, i.e.
\[
    f(M)\sim\mathcalOM{n} \;\Rightarrow\; |f(M)|<(c_f M^n) \; \forall \; M<c_0
\]
where $c_f$ and $c_0$ are constants which do not depend on M.
For our application, $c_f$ and $c_0$ may rely on any flow condition or material property other than the Mach number, although $c_0$ will usually be somewhere around 0.2, where compressibility effects become small.

In section ** we are concerned with finding (and designing) limit equations, where only the largest terms remain as $M\to0$, for which a bound is an insufficient metric.
For example, both terms in $f(M) = M^3 + M^2$ are $\mathcalOM{2}$ as $M\to0$ under the definition above, however only $M^2$ remains in the limit equation.
If we use $M^2$ as analogous to the convection (l.h.s.) terms in a modified equation, and $M^3$ as analogous to the diffusion (r.h.s.) terms in a modified equation, then $f(M)$ has asymptotically vanishing diffusion, even though $(r.h.s)\sim\mathcal{O}(l.h.s.)$ as $M\to0$.

Instead, we will a use more restrictive definition:
\[
    f(M)\sim\mathcalOM{n} \;\Rightarrow\; |f(M)|\approx (c_f M^n) \; \forall \; M<c_0
\]
Or, more formally:
\[
    f(M) \sim \mathcalOM{n} \; \Rightarrow \; \exists \; c_f \in \mathbb{R}\; \textrm{s.t.}\; \forall \varepsilon>0 \;\exists\; \delta>0 \;\textrm{s.t.}\; | f(M) - c_f M^n |<\varepsilon \; \forall \: M<\delta
\]
Which can be read as: if $f(M)\sim\mathcalOM{n}$, then $f(M)$ can be made arbitrarily close to the function $c_f M^n$ for some constant $c_f$ by simply taking M small enough.

We will also (mis-)use the \textit{less-than-approximately} and \textit{greater-than-approximately} symbols to mean, respectively, \textit{asymptotically-less-than} or \textit{asymptotically-greater-than} in the limit as $M\to0$:
\begin{alignat*}{2}
    g(M) \lesssim \mathcalOM{n} \; & \Rightarrow \; g(M) \sim \mathcalOM{m}, \quad & m>n \\
    h(M) \gtrsim  \mathcalOM{n} \; & \Rightarrow \; h(M) \sim \mathcalOM{l}, \quad & l<n
\end{alignat*}
Lastly, where terms are independent of $M$ we use $\mathcalOM{0}$ instead of $\mathcal{O}(1)$, to be clear we do not mean that the order of magnitude is necessarily on the order of unity.
